HW/SW Codesign for Robust and Efficient Binarized SNNs by Capacitor Minimization

Using accelerators based on analog computing is an efficient way to process the immensely large workloads in Neural Networks (NNs). One example of an analog computing scheme for NNs is Integrate-and-Fire (IF) Spiking Neural Networks (SNNs). However, to achieve high inference accuracy in IF-SNNs, the analog hardware needs to represent current-based multiply-accumulate (MAC) levels as spike times, for which a large membrane capacitor needs to be charged for a certain amount of time. A large capacitor results in high energy use, considerable area cost, and long latency, constituting one of the major bottlenecks in analog IF-SNN implementations. In this work, we propose a HW/SW Codesign method, called CapMin, for capacitor size minimization in analog computing IF-SNNs. CapMin minimizes the capacitor size by reducing the number of spike times needed for accurate operation of the HW, based on the absolute frequency of MAC level occurrences in the SW. To increase the operation of IF-SNNs to current variation, we propose the method CapMin-V, which trades capacitor size for protection based on the reduced capacitor size found in CapMin. In our experiments, CapMin achieves more than a 14$\times$ reduction in capacitor size over the state of the art, while CapMin-V achieves increased variation tolerance in the IF-SNN operation, requiring only a small increase in capacitor size.

==> figures/a_e_l/area.tex <==
% \begin{tikzpicture}
%     %enlargelimits=0.20,
%     %ymin=10,
% \begin{axis}[
\nextgroupplot[
	bar width=12.5,
    % ybar=0.2,
    ybar,
    bar shift=0,
    % enlarge x limits={abs=0.55},
    % enlargelimits=0.05,
    ymin=0,
    ymax=140,
    % scaled y ticks={real:0.001},
    xmin = 0,
    xmax = 4,
    % xtick=data,
    ytick distance=20,
    xtick={1,2,3},
    xticklabels={
        \textbf{Baseline},
        % \textbf{Fashion},
        % \textbf{Kuzujishi},
        % \textbf{SVHN},
        % \textbf{CIFAR10},
        \textbf{CapMin},
        \textbf{CapMin-V}
    },
    % ymode=log,
    ymajorgrids=true,
    % reverse legend=true,
    % xticklabels from table={area-new.dat}{Label},
    xticklabel style={text width=2cm,align=center},
    ylabel=Capacitance ($\SI{}{{\pico \farad}}$),
    % xticklabel style={font=\scriptsize,},
    xlabel near ticks,
    ylabel near ticks,
    ylabel shift = -0.15cm,
    height=\figureHeightB cm,
    width=\figureWidthB cm,
    nodes near coords align={vertical},
    x tick label style={rotate=30,anchor=east},
    xticklabel style={align=right, text width=2cm, font=\scriptsize, yshift={-0.1cm}},
    xtick pos=bottom,
    yticklabel style = {font=\small},
]

% % SOTA VGG3
% \addplot[draw=black,fill=000000]coordinates{(1,2472954.88)};

\addplot[draw=black,fill=000000]coordinates{(1,135.2)};

% \addplot[draw=black,fill=red]coordinates{(2,3.205)};

% \addplot[draw=black,fill=red]coordinates{(3,1.735)};

% \addplot[draw=black,fill=red]coordinates{(4,3.94)};

\addplot[draw=black,fill=2CA02C]coordinates{(2,9.575)};

\addplot[draw=black,fill=CC00FF]coordinates{(3,12.27)};

% % LTA VGG3
% \addplot[draw=black,fill=2CA02C]coordinates{(2,5070)};
% % LTA VGG3-MU
% \addplot[draw=black,fill=CC00FF]coordinates{(3,5538)};
% % SOTA VGG7
% \addplot[draw=black,fill=000000]coordinates {(4,32274000.64)};
% % LTA VGG7
% \addplot[draw=black,fill=2CA02C]coordinates{(5,49310.98)};
% % LTA VGG7-MU
% \addplot[draw=black,fill=CC00FF]coordinates{(6,49466.98)};


% \end{axis}
% \end{tikzpicture}
%\end{document}



==> figures/a_e_l/energy.tex <==
% \begin{tikzpicture}
%     %enlargelimits=0.20,
%     %ymin=10,
% \begin{axis}[
\nextgroupplot[
	bar width=12.5,
    % ybar=0.2,
    ybar,
    bar shift=0,
    % enlarge x limits={abs=0.55},
    % enlargelimits=0.05,
    ymin=0,
    ymax=1.5e-10,
    % scaled y ticks={real:0.001},
    xmin = 0,
    xmax = 4,
    % xtick=data,
    ytick distance=2e-11,
    xtick={1,2,3},
    xticklabels={
        \textbf{Baseline},
        % \textbf{Fashion},
        % \textbf{Kuzujishi},
        % \textbf{SVHN},
        % \textbf{CIFAR10},
        \textbf{CapMin},
        \textbf{CapMin-V}
    },
    % ymode=log,
    % ymajorgrids=true,
    % reverse legend=true,
    % xticklabels from table={area-new.dat}{Label},
    xticklabel style={text width=2cm,align=center},
    ylabel=Energy ($\SI{}{{\nano \joule}}$),
    % xticklabel style={font=\scriptsize,},
    xlabel near ticks,
    ylabel near ticks,
    ylabel shift = -0.15cm,
    height=\figureHeightB cm,
    width=\figureWidthB cm,
    nodes near coords align={vertical},
    x tick label style={rotate=30,anchor=east},
    xticklabel style={align=right, text width=2cm, font=\scriptsize, yshift={-0.1cm}},
    xtick pos=bottom,
]

% % SOTA VGG3
% \addplot[draw=black,fill=000000]coordinates{(1,2472954.88)};

\addplot[draw=black,fill=000000]coordinates{(1,1.352e-10)};

% \addplot[draw=black,fill=red]coordinates{(2,3.205)};

% \addplot[draw=black,fill=red]coordinates{(3,1.735)};

% \addplot[draw=black,fill=red]coordinates{(4,3.94)};

\addplot[draw=black,fill=red]coordinates{(2,9.575e-12)};

\addplot[draw=black,fill=green]coordinates{(3,1.227e-11)};

% % LTA VGG3
% \addplot[draw=black,fill=2CA02C]coordinates{(2,5070)};
% % LTA VGG3-MU
% \addplot[draw=black,fill=CC00FF]coordinates{(3,5538)};
% % SOTA VGG7
% \addplot[draw=black,fill=000000]coordinates {(4,32274000.64)};
% % LTA VGG7
% \addplot[draw=black,fill=2CA02C]coordinates{(5,49310.98)};
% % LTA VGG7-MU
% \addplot[draw=black,fill=CC00FF]coordinates{(6,49466.98)};


% \end{axis}
% \end{tikzpicture}
%\end{document}

==> figures/a_e_l/energy_multi.tex <==
%\documentclass{standalone}
%\usepackage{tikz,pgfplots,pgfplotstable}
%\pgfplotsset{compat=1.9} % set to 1.8 to get old behaviour
%%        legend style={cells={anchor=west}, legend pos=north west},
%\begin{document}
% https://tex.stackexchange.com/questions/411600/pgfplot-tikz-stacked-bar-chart-with-compat-1-9-or-later
%\pgfplotstableread{
%Label   series1 series2 series3
%4\ bits\ Model  10000   1  1
%BNN\ w\ BETT    1    100    1
%BNN\ w/o\ BETT  1   1   125
%}\testdata



\begin{tikzpicture}
    %enlargelimits=0.20,
    %ymin=10,
\begin{axis}[
	bar width=12.5,
    ybar stacked,
    enlarge x limits={abs=0.55},
    ymin=0,
    ymax=100,
    xtick=data,
    % ytick distance=50,
    reverse legend=true,
    xticklabels from table={BAR-ENG-v5.dat}{Label},
    xticklabel style={text width=2cm,align=center},
    ylabel=Energy (nJ),
    xticklabel style={font=\scriptsize,},
    legend style={nodes={scale=0.65, transform shape}},
    legend columns=3,
    %xticklabel style={align=right, text width=2cm, font=\scriptsize, yshift={-0.1cm}, rotate=45, anchor=east},
    height=\figureHeight cm,
    width=\figureWidth cm
]

\addplot [fill=magenta] table [y=Counter, x expr=\coordindex] {BAR-ENG-v5.dat};
%\addlegendentry{Counter}
%\addlegendentry{4\ bits\ Model}
%
\addplot [fill=B22222] table [y=Reciprocal, x expr=\coordindex] {BAR-ENG-v5.dat};
\addlegendentry{Time-to-digit}
%
\addplot [fill=yellow] table [y=Adder, x expr=\coordindex] {BAR-ENG-v5.dat};
\addlegendentry{Adder}

%
%
\addplot [fill=00C8C8] table [y=Crossbar, x expr=\coordindex] {BAR-ENG-v5.dat};
\addlegendentry{Cros.+Neuron}

\addlegendentry{Counter}
\addplot [fill=magenta,nodes near coords,point meta=y,nodes near coords style={anchor=south}] table [y=topple, meta=Label, x expr=\coordindex] {BAR-ENG-v5.dat};

%\addlegendentry{BNN\ w/o\ BETT}

\end{axis}
\end{tikzpicture}
%\end{document}

%Label           Counter       A      Crossbar  Reciprocal       RNG       topper
%4-bits          560           40     101120    27520            54000     183240
%BNN             7             40     64000      27520            675       92242
%BNN-ERT         5.6           40     50560      27520            540       78665.6%

==> figures/a_e_l/latency.tex <==
% \begin{tikzpicture}
%     %enlargelimits=0.20,
%     %ymin=10,
% \begin{axis}[
\nextgroupplot[
	bar width=12.5,
    % ybar=0.2,
    ybar,
    bar shift=0,
    % enlarge x limits={abs=0.55},
    % enlargelimits=0.05,
    ymin=0,
    ymax=400,
    % scaled y ticks={real:0.001},
    xmin = 0,
    xmax = 4,
    % xtick=data,
    ytick distance=50,
    xtick={1,2,3},
    xticklabels={
        \textbf{Baseline},
        % \textbf{Fashion},
        % \textbf{Kuzujishi},
        % \textbf{SVHN},
        % \textbf{CIFAR10},
        \textbf{CapMin},
        \textbf{CapMin-V}
    },
    % ymode=log,
    ymajorgrids=true,
    % reverse legend=true,
    % xticklabels from table={area-new.dat}{Label},
    xticklabel style={text width=2cm,align=center},
    ylabel=Latency ($\SI{}{{\nano \second}}$),
    % xticklabel style={font=\scriptsize,},
    xlabel near ticks,
    ylabel near ticks,
    ylabel shift = -0.15cm,
    height=\figureHeightB cm,
    width=\figureWidthB cm,
    nodes near coords align={vertical},
    x tick label style={rotate=30,anchor=east},
    xticklabel style={align=right, text width=2cm, font=\scriptsize, yshift={-0.1cm}},
    xtick pos=bottom,
    yticklabel style = {font=\small}
]

% % SOTA VGG3
% \addplot[draw=black,fill=000000]coordinates{(1,2472954.88)};

\addplot[draw=black,fill=000000]coordinates{(1,357.5)};

% \addplot[draw=black,fill=red]coordinates{(2,3.205)};

% \addplot[draw=black,fill=red]coordinates{(3,1.735)};

% \addplot[draw=black,fill=red]coordinates{(4,3.94)};

\addplot[draw=black,fill=2CA02C]coordinates{(2,25.5)};

\addplot[draw=black,fill=CC00FF]coordinates{(3,32.5)};

% % LTA VGG3
% \addplot[draw=black,fill=2CA02C]coordinates{(2,5070)};
% % LTA VGG3-MU
% \addplot[draw=black,fill=CC00FF]coordinates{(3,5538)};
% % SOTA VGG7
% \addplot[draw=black,fill=000000]coordinates {(4,32274000.64)};
% % LTA VGG7
% \addplot[draw=black,fill=2CA02C]coordinates{(5,49310.98)};
% % LTA VGG7-MU
% \addplot[draw=black,fill=CC00FF]coordinates{(6,49466.98)};


% \end{axis}
% \end{tikzpicture}
%\end{document}
